Parabola-Inscribed Poncelet Polygons Derived from the Bicentric Family

We study loci and properties of a Parabola-inscribed family of Poncelet polygons whose caustic is a focus-centered circle. This family is the polar image of a special case of the bicentric family with respect to its circumcircle. We describe closure conditions, curious loci, and new conserved quantities.

==> 910_app_poncelet.tex <==
\section{Poncelet's Porism}
\label{app:poncelet}

Given two real conics $\E$ and $\E'$, a {\em Poncelet transverse} is constructed as follows (see \cref{fig:poncelet}): pick a point $P_1$ on $\E$ and shoot a ray in the direction of one of the tangents to $\E'$. Let $P_2$ denote the non-$P_1$ intersection of this ray with $\E$, i.e., $P_1 P_2$ is a chord of $\E$. Now shoot a ray from $P_2$ in the direction of a tangent to $\E'$ and find $P_3$, etc., repeating this a number of times. For certain conic pairs, the transverse closes after $N$ steps, i.e., $P_N=P_1$. Pairs with this property are said to satisfy ``Cayley's conditions'', see \cite{dragovic11} details.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_01_005_poncelet}
    \caption{\textbf{Top left}: 3 Poncelet iterations within a pair of ellipses in general position; their centers are labeled $O$ and $O_c$, respectively. \text{Top right:} 5 more iterations executed (starting at $P_4$), showing the trajectory is not likely to close. \textbf{Bottom:} a new ellipse pair for which an iteration departing from $P_1$ closes after 7 steps (blue polygon). Poncelet's porism guarantees that if the iteration were to start anywhere else on the outer ellipse, e.g., $P_1'$, it will also yield a closed, 7-gon (dashed red). \href{https://youtu.be/kzxf7ZgJ5Hw}{Video},  \href{https://observablehq.com/@dan-reznik/poncelet-iteration}{Live}}
    \label{fig:poncelet}
\end{figure}

Poncelet's closure theorem (PCT) states that if such an $N$-step transverse closes, than one that starts from any other point on $\E$ will also close in $N$ steps, i.e., one has a 1d family of Polygons \cite{centina15}. 

In the specific case where $\E$ and $\E'$  are concentric, axis-aligned ellipses, the Cayley condition for such a pair to admit a family of triangles reduces to   \cite{georgiev2012-poncelet}:

\[ \frac{a'}{a} + \frac{b'}{b} = 1 \]
where $a,b$ (resp. $a',b'$) are the semiaxes of $\E$ (resp. $\E'$).

A few such pairs are shown in \cref{fig:six-caps}. These include a pair (i) with a fixed incircle (and external ellipse), (ii) a fixed circumcircle (and internal inellipse), (iii) of homothetic ellipses, (iv) of ``dual'' ellipses (these have reciprocal aspect ratios), and (v) of the {\em excentral} triangles\footnote{The excentral triangle has sides through the vertices of a reference one and along the external bisectors.} to the confocal pair itself.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_01_050_six_caps_perp}
    \caption{The confocal family is shown at the top left. Also shown are 5 other ``famous'' concentric families. \href{https://youtu.be/14TQ5WlZxUw}{Video}}
    \label{fig:six-caps}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics/pics_00_020_poristic_brocard}
    \caption{The poristic family (left), also known as Bicentric triangles, and the Brocard porism (right), also known as harmonic triangles.}
    \label{fig:por-broc}
\end{figure}

==> refs_rgk_media.tex <==
@MISC{impa2019,
   author = {Dan Reznik and Ronaldo Garcia and Jair Koiller},
   title = {Adventures with Triangles and Billiards},
   url={impa.br/en_US/eventos-do-impa/eventos-2019/ 32o-coloquio-brasileiro-de-matematica},
   address={Rio de Janeiro},
   institution = {Instituto Nacional de    Matemática Pura e Aplicada (IMPA)},
   day={31},
   month={7},
   year={2019},
}

@MISC{impa2019_video,
   author = {Dan Reznik and Ronaldo Garcia and Jair Koiller},
   title = {Adventures with Triangles and Billiards},
   url={youtu.be/t872mftaI2g},
   publisher={YouTube},
   day={15},
   month={8},
   year={2019},
}

@MISC{reznik_web,
   author = {Dan Reznik and Ronaldo Garcia and Jair Koiller},
   title={New Properties of Triangular Orbits in Elliptic Billiards},
   url={dan-reznik.github.io/Elliptical-Billiards-Triangular-Orbits/},
   year={2019}
}

@MISC{reznik_media,
   author = {Dan Reznik and Ronaldo Garcia and Jair Koiller},
   title={Media for Elliptic Billards and Family of Orbits},
   url={dan-reznik.github.io/Elliptical-Billiards-Triangular-Orbits/videos.html},
   year={2019}
}

@MISC{reznik_loci,
   author = {Dan Reznik},
   title={Triangular Orbits in Elliptic Billards: Loci of Points {X}(1)~{X}(100)},
   url={dan-reznik.github.io/Elliptical-Billiards-Triangular-Orbits/loci_6tri.html},
   year={2019}
}

@MISC{dsr_vid11incenter,
  author={Dan Reznik},
  title={Triangular Orbits in Elliptic Billiards: Locus of the Incenter is an Ellipse},
  year={2011},
  url={youtu.be/9xU6T7hQMzs},
  publisher={YouTube}
}

@MISC{dsr_vid11e,
  author={Dan Reznik},
  title={Locus of the incircle touchpoints is a higher-order curve},
  year={2011},
  url={youtu.be/9xU6T7hQMzs},
  publisher={YouTube}
}

@MISC{dsr_applet11a,
  author={Dan Reznik},
  title={"Dynamic Billiards in Ellipse"},
  url={demonstrations.wolfram.com/DynamicBilliardsInEllipse/},
  publisher={Wolfram Demonstrations Project},
  year={2011}
}

@MISC{playlist2020-deltoid,
author={Dan Reznik},
  title={{YouTube} Playlist for Constant-Area Deltoid},
  year={2020},
  publisher={YouTube},
  url={bit.ly/3gqfIRm}
}

@MISC{dsr_main_videos_2019,
  author={Dan Reznik},
  title={New Properties of Polygonal Orbits in Elliptic Billiards: Main Videos},
  year={2019},
  url={bit.ly/2k5GXbB},
  publisher={YouTube}
}

@MISC{dsr_playlist_2020,
  author={Dan Reznik},
  title={Playlist for {``Loci of Triangular Orbits in an Elliptic Billiard''}},
  year={2020},
  url={bit.ly/3072LV3},
  publisher={YouTube}
}

@MISC{dsr_playlist_2020_proofs,
  author={Dan Reznik},
  title={Playlist for {``New Properties of Triangular Orbits in an Elliptic Billiard''}},
  year={2020},
  url={bit.ly/379mk1I},
  publisher={YouTube}
}

@MISC{dsr_playlist_2020_polygons,
  author={Dan Reznik},
  title={Playlist for {``Invariants of N-Periodics in the Elliptic Billiard''}},
  year={2020},
  url={bit.ly/2xeVGYw},
  publisher={YouTube}
}

@MISC{dsr_playlist_2020_invariants,
  author={Dan Reznik},
  title={Playlist for {``Invariants of N-Periodic Trajectories in Elliptic Billiards''}},
  year={2020},
  url={bit.ly/3aNqgqU},
  publisher={YouTube}
}


@MISC{dsr_locus_gallery_2019,
  author={Dan Reznik},
  title={Triangular Orbits in Elliptic Billards: Loci of Points {X(1)~X(100)}},
  year={2019},
  url={dan-reznik.github.io/Elliptical-Billiards-Triangular-Orbits/loci_6tri.html},
  publisher={GitHub}
}

@MISC{dsr_applet_x12345,
author={Dan Reznik},
  title={Applet Showing the Locus of Several Triangular Centers},
  year={2019},
  publisher={P5.js},
  url={editor.p5js.org/dreznik/full/i1Lin7lt7}
}

@MISC{darlan2020-app,
author={Iverton Darlan and Dan Reznik},
title={Loci of Ellipse-Mounted Triangle Centers},
year={2020},
url={dan-reznik.github.io/ellipse-mounted-triangles/}
}

@MISC{sundrop2016,
author={Sundrop Farms},
title={February 2016 Update},
howpublished={{YouTube}},
year={2016},
url={https://youtu.be/rRNy89j6wMc}
}

@MISC{esolar2017,
author={General Electric},
title={{eSolar} Concentrated Solar plants},
howpublished={{YouTube}},
year={2017},
url={https://youtu.be/ADbUsuNeRQE}
}

@MISC{garcia2021-ellipses-web,
author={Ronaldo Garcia and Dan Reznik and Jair Koiller},
  title={Companion Website to ``Loci of 3-periodics in an Elliptic Billiard: Why so many ellipses?''},
  month={1},
  year={2021},
  howpublished={{GitHub Pages}},
  url={dan-reznik.github.io/why-so-many-ellipses/}
}

@MISC{reznik2021-observable-media,
author={Dan Reznik},
  title={Experimental {P}oncelet Media Assets},
  month={5},
  year={2021},
  howpublished={{Observable}},
  url={https://observablehq.com/@dan-reznik/poncelet-media-assets}
}

@MISC{reznik2021-observable-poncelet-closure,
author={Dan Reznik},
  title={{P}oncelet's Closure Theorem},
  month={5},
  year={2021},
  howpublished={{Observable}},
  url={https://observablehq.com/@dan-reznik/poncelet-iteration}
}

@MISC{reznik2021-observable-jacobi-elliptic-fns,
author={Dan Reznik},
  title={Jacobi's complete integral of first kind and elliptic functions},
  month={5},
  year={2021},
  howpublished={{Observable}},
  url={https://observablehq.com/@dan-reznik/jacobi-elliptic-functions}
}

@MISC{reznik2021-observable-spatiotemporal,
author={Claudio Esperança and Ronaldo Garcia and Dan Reznik},
  title={Elliptic Billiard 3-Periodics & Spatio-Temporal Visualization},
  month={5},
  year={2021},
  howpublished={{Observable}},
  url={https://observablehq.com/@dan-reznik/elliptic-billiard-triangle}
}

@misc{reznik2021-artful,
author={Dan Reznik},
Title={Arful Loci of Triangles in Ellipses},
year={2021},
howepublished={{Google Slides}},
url={https://bit.ly/34sO8Px}
}

@MISC{reznik2021-locus-app-tutorial,
title={Locus App Tutorial: a Video Walkthrough},
author={Dan Reznik},
year={2021},
howpublished={{YouTube}},
url={https://bit.ly/3iCKHxn}
}
